KC-Bench: A Dynamic Interactive Benchmark for Evaluating Knowledge Conflicts in LLM Agents

As LLMs increasingly act through tools, they must reconcile user instructions, parametric knowledge, and dynamic environmental observations before taking actions. We introduce KC-Bench, a controlled multi-turn benchmark for measuring this capability across world-knowledge conflicts, input inconsistencies, and multi-source temporal conflicts. Its 238 tasks are manually screened from more than 1,000 generated candidates and combine a user simulator, stateful tools, deterministic environment assertions, an open-source natural-language evaluator, and human trajectory verification. Evaluation of nine models, including DeepSeek-V4-Flash, GLM-5.2, and MiniMax-M3, shows substantial cross-domain variation: no model handles factual correction, identity consistency checking, and temporal conflict resolution reliably across all settings. In the simulated environments, missed conflicts can propagate to tool calls or synthetic protected-data flows. KC-Bench isolates this model-level behavior rather than ranking complete agent frameworks, and provides a reproducible diagnostic for developing conflict-aware reasoning and execution safeguards.

==> Section/limitation.tex <==
\section{Limitations}
KC-Bench isolates conflict handling in a standardized lightweight harness; it does not evaluate complete agent products with persistent memory, skill management, planning, recovery, or additional guardrails. Such framework components may materially change behavior. The 238 retained tasks are a manually screened subset of more than 1,000 generated candidates across three simulated domains, so they support comparisons within the tested conflict mechanisms rather than broad claims about all deployment settings. Each distinct task is executed once with temperature 0 and a fixed seed. This reduces generation variance but does not quantify sensitivity to alternative system prompts or stochastic decoding; conservative safety prompts are an important intervention for future study. Human verification corrects limitations of the natural-language evaluator, but no blind human-agent performance baseline or inter-annotator agreement statistic is reported. Finally, simulated disclosure or unsafe execution indicates a potential failure mode, not a real privacy incident, legal violation, or proof about a model's training method. Production authentication and authorization must be enforced by deterministic system-level controls.

